ColA: Collaborative Adaptation with Gradient Learning

A primary function of back-propagation is to compute both the gradient of hidden representations and parameters for optimization with gradient descent. Training large models requires high computational costs due to their vast parameter sizes. While Parameter-Efficient Fine-Tuning (PEFT) methods aim to train smaller auxiliary models to save computational space, they still present computational overheads, especially in Fine-Tuning as a Service (FTaaS) for numerous users. We introduce Collaborative Adaptation (ColA) with Gradient Learning (GL), a parameter-free, model-agnostic fine-tuning approach that decouples the computation of the gradient of hidden representations and parameters. In comparison to PEFT methods, ColA facilitates more cost-effective FTaaS by offloading the computation of the gradient to low-cost devices. We also provide a theoretical analysis of ColA and experimentally demonstrate that ColA can perform on par or better than existing PEFT methods on various benchmarks.

==> analysis.tex <==
% The following analysis is for a more general case left for future writeup. For now we use a simplified version and comment it
\subsection{Theoretical Analysis}


Suppose $g_m$ is restricted to a linear function. Suppose the initial parameter of the pre-trained model is $\th$. Let $\E_n f(x) $ denote the empirical average $n^{-1} \sum_{i=1}^n f(x)$ for any function $f$. Let $V_m \de \E_n \{x_m x_m^\T\}$ be the empirical covariance matrix of the input of layer $m$. Let $U_m \de V_m^{-1/2}$ denote the matrix that satisfies $U_m^\T U_m = V_m^{-1}$.

For each training iteration $t=1,\ldots,T$: 

% the following version is the utmost simplified version that f is also linear. But this is not necessary for the proof to hold
% $\bullet$ Compute forward pass and gather input-output for a generic input $x$ at layer $m$ as: $(x_m, \hat{h}_m)$, where $\hat{h}_m = h_m + g_m^{t}(x_m)$, where $h_m \de f_{\th_m}(x_m) = \th_m x_m$ and $g_m^{t}(x_m) \de w_m^{t} x$. Thus, we have $\hat{h}_m = (\th_m +w_m^{t}) x_m = f_{\th_m+w_m^{t}}(x_m)$. Let $w^{t}=\cup_{m \in [M]} w_m^{t}$, like how $\th$ is defined. So, the updated global model at round $t$ would be parameterized by $\th + w^{t}$, namely $x \mapsto f_{\th, w^{t}}(x)$.

$\bullet$ Compute forward pass and gather input-output for a generic input $x$ at layer $m$ as: $(x_m, \hat{h}_m(x_m))$, where $\hat{h}_m(x_m) = h_m(x_m) + g_m(x_m)$, where $h_m(x_m) \de f_{\th_m}(x_m)$ and we parameterize $g_m(x) = w_m U_m  x$. 
%we parameterize $g_m(x) \de  q(w_m) \cdot x$, where $q$ is any function that maps the learnable parameter $w_m$ to a matrix of dimension $\R^{d_{m,\texttt{in}} \times d_{m,\texttt{out}}}$. 
At round $t$, we write $g_m^{t}(x_m) \de w_m^{t} U_m x_m$. Let $w^{t}=\cup_{m \in [M]} w_m^{t}$. The updated global model at round $t$ is represented by $f_{\th,w^t}(x_m)$.


$\bullet$ Gather the gradient of the loss with respect to layer $m$'s output, $\nabla_{\hat{h}_m}  \ell(y, f_{\th, w^{t}}(x))$.

$\bullet$ Prepare adaptation data, which are input-output pairs in the form of $(x, z_m^t)$, where 
\begin{align}   
    z_m^t \de g_m^{t}(x_m) - \gamma_t \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x)). \label{eq_1} 
\end{align}
$\bullet$ Run $A$ iterations to update from $g_m^{t}$ to $g_m^{t+1}$ by minimizing $\E_n \norm{ g_m(x) - z_m^t }^2 / 2$. 


\begin{proposition}
    The gradient update of $w_m$ in our algorithm and that of the global fine-tuning approach differs in a factor of $O(e^{-\sum_{j=1}^{A} \alpha_j})$, which is a term when $\sum_{j=1}^{A} \alpha_j$ diverges as $A$ goes large.
\end{proposition}

\begin{proof}
    
Since $g_m(x) = w_m U_m x$, this amounts to updating from $w_m^{t}$ to $w_m^t$ through the following sequence of updates:
\begin{align}
    w_m^{t,0} 
    &\de w_m^{t}, \textrm{ and for } \ell = 1, \ldots, \NA, \\
    w_m^{t,\ell} 
    &= w_m^{t,\ell-1} - \alpha_{\ell} \cdot \nabla_{w_m} \E_n  \biggl\{\norm{w_m^{t,\ell-1} U_m x_m - z_m^t}^2 /2  \biggr\}\\
    &= w_m^{t,\ell-1} - \alpha_{\ell} \cdot \E_n \biggl\{ (w_m^{t,\ell-1} U_m x_m - z_m^t) x_m^\T U_m^\T \biggr\} \label{eq_2}
\end{align}
Bringing (\ref{eq_1}) into (\ref{eq_2}), we obtain 
\begin{align*}
    w_m^{t,\ell} 
    &= w_m^{t,\ell-1} - \alpha_{\ell} \cdot \E_n \biggl\{ (w_m^{t,\ell-1} U_m x_m - g_m^{t}(x_m) + \gamma_t \cdot \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\} \\
    &= w_m^{t,\ell-1} - \alpha_{\ell} \cdot \E_n \biggl\{ (w_m^{t,\ell-1} U_m x_m - w_m^{t} U_m x_m + \gamma_t \cdot \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\} \\
    &= w_m^{t,\ell-1} - \alpha_{\ell} \cdot (w_m^{t,\ell-1}- w_m^{t}) U_m \E_n \{ x_m  x_m^\T\} U_m^\T  - \alpha_{\ell} \cdot \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\} \\
    &= w_m^{t,\ell-1} - \alpha_{\ell} \cdot (w_m^{t,\ell-1}- w_m^{t}) - \alpha_{\ell} \cdot \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m}  \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T  U_m^\T \biggr\} 
\end{align*}
Subtracting $c_m^{t} \de w_m^{t} - \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\}  $ in both sides of the above equation, we obtain
\begin{align}
    w_m^{t,\ell} - c_m^{t} = (1 - \alpha_{\ell} ) (w_m^{t,\ell-1} - c_m^{t})  . \label{eq_3}
\end{align}
 By recursively applying (\ref{eq_3}) for $\ell=1,\ldots,\NA$, we have
\begin{align}
    w_m^{t,\ell} - c_m^{t} 
    &= (w_m^{t,0} - c_m^{t}) \cdot \prod_{j=1}^{\ell} (1 - \alpha_{j}) \\
    &= \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\}  \cdot \prod_{j=1}^{\ell}(1 - \alpha_{j}),
\end{align}
which implies that
\begin{align}
    w_m^{t+1}  
    =& w_m^{t} - \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m}  \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\}   \nonumber \\
    &+ \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\}  \cdot \prod_{j=1}^{A} (1 - \alpha_{j}) \label{eq_4}
\end{align}
Since
\begin{align*}
     \prod_{j=1}^{A} (1 - \alpha_{j})  
    & = \exp\biggl(\sum_{j=1}^{A} \log(1-\alpha_j ) \biggr) \\
    &\leq \exp\biggl( -\sum_{j=1}^{A} \alpha_j \biggr),
\end{align*}
we have 
\begin{align}
    w_m^{t+1}  
    =& w_m^{t} - \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m}  \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\} (1+O(e^{-\sum_{j=1}^{A} \alpha_j})) \label{eq_6}
\end{align}
%
% THe following is unnormalized version
% \begin{align}
%     w_m^{t,\ell} - c_m^{t} = (w_m^{t,\ell-1} - c_m^{t}) \cdot (I - \alpha_{\ell} V_m), \label{eq_3}
% \end{align}
% where $I$ is a matrix whose dimension matches that of $x_m$. By recursively applying (\ref{eq_3}) for $\ell=1,\ldots,\NA$, we have
% \begin{align}
%     w_m^{t,\ell} - c_m^{t} 
%     &= (w_m^{t,0} - c_m^{t}) \cdot \prod_{j=1}^{\ell} (I - \alpha_{j} V_m) \\
%     &= \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\}  \cdot V_m^{-1} \cdot \prod_{j=1}^{\ell} (I - \alpha_{j} V_m),
% \end{align}
% which implies that
% \begin{align}
%     w_m^{t+1}  
%     =& w_m^{t} - \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m}  \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\}  \cdot V_m^{-1} \nonumber \\
%     &+ \gamma_t \cdot \E_n \biggl\{ \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x))) \cdot x_m^\T U_m^\T \biggr\}  \cdot V_m^{-1}  \cdot \prod_{j=1}^{A} (I - \alpha_{j} V_m) \label{eq_4}
% \end{align}
%
% Suppose the smallest eigenvalue of $\E_n \{x_m x_m^\T\}$ is $\lambda_m > 0$. we have 
% \begin{align*}
%     \bnorm{\prod_{j=1}^{A} (I - \alpha_{j} V_m)} 
%     &\leq \prod_{j=1}^{A} \norm{I - \alpha_{j} V_m} \\
%     &\leq \prod_{j=1}^{A} (1-\alpha_j \lambda_m) = \exp\biggl(\sum_{j=1}^{A} \log(1-\alpha_j \lambda_m) \biggr) \\
%     &\leq \exp\biggl( -\sum_{j=1}^{A} \alpha_j \lambda_m \biggr).
% \end{align*}
%
 
On the other hand, if we run standard gradient descent, we would have the update: 
\begin{align}   
    w_m^{t+1} 
    &=w_m^{t} - \eta_t \cdot \nabla_{w} \E_n \ell(y, f_{\th, w^{t}}(x)) \\
    &=w_m^{t} - \eta_t \cdot \E_n \{\nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x)) \cdot (\nabla_{w} \hat{h}_m)^\T \} \\
    &=w_m^{t} - \eta_t \cdot \E_n \{\nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x)) \cdot (\nabla_{w} g_m^{t}(x_m))^\T \} \\
    &=w_m^{t} - \eta_t \cdot \E_n \{ \nabla_{\hat{h}_m} \ell(y, f_{\th, w^{t}}(x)) \cdot x_m^\T \} \label{eq_5} 
\end{align}
Comparing (\ref{eq_6}) and (\ref{eq_5}), one can see that the difference of the gradient update is up to a factor of $O(e^{-\sum_{j=1}^{A} \alpha_j})$, which is a term when $\sum_{j=1}^{A} \alpha_j$ diverges as $A$ goes large.

\end{proof}
